On Improved Regret Bounds In Bayesian Optimization with Gaussian Noise

Bayesian optimization (BO) with Gaussian process (GP) surrogate models is a powerful black-box optimization method. Acquisition functions are a critical part of a BO algorithm as they determine how the new samples are selected. Some of the most widely used acquisition functions include upper confidence bound (UCB) and Thompson sampling (TS). The convergence analysis of BO algorithms has focused on the cumulative regret under both the Bayesian and frequentist settings for the objective. In this paper, we establish new pointwise bounds on the prediction error of GP under the frequentist setting with Gaussian noise. Consequently, we prove improved convergence rates of cumulative regret bound for both GP-UCB and GP-TS. Of note, the new prediction error bound under Gaussian noise can be applied to general BO algorithms and convergence analysis, e.g., the asymptotic convergence of expected improvement (EI) with noise.

==> Sections/Asymptotic.tex <==
\section{Asymptotic convergence analysis}\label{se:convergence}
  In this section, we consider the asymptotic convergence behavior of the EI and the BO-EI algorithm. 
  Denote the optimal solution as $f(\xbm^*)$, we consider the error measure $r_t$ with $t$ samples by 
 \begin{equation} \label{eqn:asymp-error}
 \centering
  \begin{aligned}
       r_t = y^+_{t}-f(\xbm^*),
  \end{aligned}
\end{equation}
  which recovers $f(\xbm_t)-f(\xbm^*)$ used for asymptotic convergence analysis in~\cite{bull2011convergence} without noise. 
  We note that as in inexact optimization literautre~\cite{}, we prove the iterates generated by the algorithm converges to the vicinity of $\xbm^*$ with a high probability. 
  While~\eqref{eqn:asymp-error} is not guaranteed to be positive, $r_t\leq r_{t-1}$. The result based on~\eqref{eqn:asymp-error} can be readily used to bound $f(\xbm^+)-f(\xbm^*)$, with the addition of noise at $\xbm^+$ that generates $y^+_t$. We opt for~\eqref{eqn:asymp-error} since $y^+_t$ is the actual output of BO-EI and plays an integral part in the algorithm itself. 

  Assumption~\ref{assp:gp} and~\ref{assp:constraint} are considered valid in this section.
  We first prove a bound on $r_t$ similar to that in~\cite{bull2011convergence}. It is worth pointing out that the asymptotic convergence of BO-EI under  Assumption~\ref{assp:gp} is novel for both the noiseless and noisy cases.
   We state the straightforward result that $f$ is bounded on $C$ as a Lemma for easy reference. 
\begin{lemma}\label{lem:f-bound}
  There exists $M>0$, such that $f(\xbm)\leq M$ for all $x\in C$.
\end{lemma}
 \begin{theorem}\label{theorem:EI-convergence-1}
   Given $\delta\in(0,1)$, let $\beta=\max\{1,2 \log (2 /\delta)\}$.
   Running the BO-EI algorithm with GP prior $(0,k(\xbm,\xbm'))$ leads to the error bound  
      \begin{equation} \label{eqn:EI-convg-1}
  \centering
  \begin{aligned}
               r_t =   \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} \left[3\frac{2M+2c_\sigma \sigma}{t} +(\beta^{1/2}+0.4) \sigma_{t_k}^{\alpha}(\xbm_{t_k+1}))\right],\\
   \end{aligned}
  \end{equation} 
 where $t/3-1\leq t_k\leq t$, with probability $\geq 1-2\Phi(-c_\sigma)-\delta-(\frac{1}{2})^{t/3}$
\end{theorem}
\begin{proof}
   Since $y_t = f(\xbm_t) + \epsilon_t$ and $\epsilon_t\sim\mathcal{N}(0,\sigma^2)$, with probability $\geq 1-\Phi(-c_{\sigma})$, 
  \begin{equation} \label{eqn:EI-convg-pf-0.5}
  \centering
  \begin{aligned}
        y_t - f(\xbm_t) \leq c_{\sigma}\sigma, 
  \end{aligned}
  \end{equation}
 for $\forall t\in\Nbb$, where $c_{\sigma}>0$ is a constant. Therefore, with probability $\geq 1-\Phi(-c_{\sigma})$, 
  \begin{equation} \label{eqn:EI-convg-pf-1}
  \centering
  \begin{aligned}
        y^+_{t}- f(\xbm_{t+1}) \leq y^+_{t}-y_{t+1}+c_{\sigma}\sigma \leq y^+_{t}-y^+_{t+1} + c_{\sigma} \sigma . 
  \end{aligned}
  \end{equation}
  Similarly, with probability $1-\Phi(-c_{\sigma})$, $y_t-f(\xbm_t)\geq -c_{\sigma}\sigma$. 
  Moreover, from Lemma~\ref{lem:f-bound},~\eqref{eqn:EI-convg-pf-0.5}, and union bound, with probability $\geq 1-2\Phi(-c_{\sigma})$,
  \begin{equation} \label{eqn:EI-convg-pf-2}
  \centering
  \begin{aligned}
        \sum_{t=0}^{T-1}  y^+_{t}-y^+_{t+1} = y^+_0 - y_T^+ \leq 2 M +2c_{\sigma}\sigma. 
  \end{aligned}
  \end{equation}
  Given that $y^+_{t}-y^+_{t+1}\geq 0$, $y^+_{t}-y^+_{t+1} \geq \frac{2M +2c_{\sigma}\sigma}{k}$ at most $k$ times for any $k\in \Nbb$. 

  
  Consider first the noiseless case where $\sigma=0$. 
  Choose $k=[t/2]$, where $[x]$ is the largest integer smaller than $x$. Then, $2k\leq t\leq 2(k+1)$.
  Then , there exists $k\leq t_k\leq 2k$ so that $y^+_{t_k}-y^+_{t_k+1} < \frac{2M}{k}$. 
   Since $\{y^+_t\}$ is monotonically non-increasing, using $\delta/2$ and $t_k$ in Lemma~\ref{lem:IEIbound-ratio}, we have with probability $\geq 1-\delta/2$, 
  \begin{equation} \label{eqn:EI-convg-pf-3}
  \centering
  \begin{aligned}
          r_t =& y^+_{t}-f(\xbm^*)
                  \leq y^+_{t_k}-f(\xbm^*) \leq I_{t_k}(\xbm^*) \\
                  \leq& \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} EI_{t_k}(\xbm^*,\alpha) 
                  \leq \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} EI_{t_k}(\xbm_{t_k+1},\alpha) \\
                  =& \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} (y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+\sigma_{t_k}^{\alpha}\phi(z_{t_k}(\xbm_{t_k+1},\alpha)) \\
  \end{aligned}
  \end{equation}
  Given no noise, $y^+_{t}\leq f(\xbm_t)$ for all $t\in\Nbb$. Thus, by using $\delta/2$ and $t_k$ in Lemma~\ref{lem:fmu-alpha}, we have 
  \begin{equation} \label{eqn:EI-convg-pf-3.5}
  \begin{aligned}
  \centering
   y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1})=&y^+_{t_k}-y^+_{t_k+1}+y^+_{t_k+1}-f(x_{t_k+1})+f(x_{t_k+1})-\mu_{t_k}(\xbm_{t_k+1})\\
   <& \frac{2M}{k} + f(\xbm_{t_k+1})-\mu_{t_k}(\xbm_{t_k+1})\leq \frac{2M}{k}+\beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}).
   \end{aligned}
  \end{equation}
   From~\eqref{eqn:EI-convg-pf-3.5} and Lemma~\ref{lem:phi},~\eqref{eqn:EI-convg-pf-3} is simplified to   
  \begin{equation} \label{eqn:EI-convg-pf-4}
  \centering
  \begin{aligned}
     r_t    \leq& \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} \left[\frac{2M }{k}+(\beta^{1/2}+0.4)\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\right].\\
  \end{aligned}
  \end{equation}


  Next, we extend the results to the noisy case. Given a sequence of iterates $\xbm_i,i\in A_k$ of size $k\in \Nbb$, \textit{i.e.}, $|A_k|=k$, the probability of $f(\xbm_i) < y_i = f(\xbm_i)+\epsilon_i$ for all $i\in A_k$ is $(\frac{1}{2})^k$, thanks to the independent distribution of $\epsilon_i$. Equivalently, the probability that there exists a $i\in A_k$ such that $f(\xbm_i)\geq y_i$ is $1-(\frac{1}{2})^k$.
  Let $k=[t/3]$. Then, $3k\leq t\leq 3(k+1)$.
  There exists $k \leq t_k \leq 3k$ so that $y_{t_k}^+-y_{t_k+1}^+<\frac{2M+2c_{\sigma}\sigma}{k}$ and $f(\xbm_{t_k+1})\geq y_{t_k+1}\geq y_{t_k+1}^+$ with probability $\geq 1-2\Phi(-c_{\sigma})-(\frac{1}{2})^k$.
  Using $\delta/2$ and $t_k$ in Lemma~\ref{lem:IEIbound-ratio} and~\ref{lem:fmu-alpha}, with probability $\geq 1-2\Phi(-c_{\sigma})-(\frac{1}{2})^k-\delta$, 
 \begin{equation} \label{eqn:EI-convg-pf-5}
  \centering
  \begin{aligned}
          r_t =& y^+_{t}-f(\xbm^*)\leq y^+_{t_k}-f(\xbm^*)=I_{t_k}(\xbm^*)\\ 
                  \leq& \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} EI_{t_k}(\xbm^*,\alpha) 
                  \leq \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} EI_{t_k}(\xbm_{t_k+1},\alpha) \\
                  =& \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} \left[(y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\phi(z_{t_k}(\xbm_{t_k+1},\alpha))\right] \\
                  \leq& \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} \left[\frac{2M+2c_\sigma \sigma}{k}+y_{t_k+1}^+-f(\xbm_{t_k+1})+f(\xbm_{t_k+1})-\mu_{t_k}(\xbm_{t_k+1})+0.4\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}) \right]\\
                  \leq& \frac{\tau(\beta^{1/2})}{\tau(-\beta^{1/2})} \left[\frac{2M+2c_\sigma \sigma}{k} +(\beta^{1/2}+0.4)\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\right].\\
  \end{aligned}
  \end{equation}
  The inequalities in~\eqref{eqn:EI-convg-pf-5} can be obtained in a similar fashion as those in~\eqref{eqn:EI-convg-pf-4}.
\end{proof}

Next, we give the following convergence rate by fully utilizing the properties and behavior of EI. 
\begin{theorem}\label{theorem:EI-convg-star}
   Given $\delta\in(0,0.425)$, let $\beta=\max\{1, c_{\beta}^{-1} \log (3c_{\alpha}/\delta)\}$, where $c_{\beta}=0.427,c_{\alpha}=1.09$.
   Choose the constants $C_1,C_2>0$ so that\\ 
     (a) $\left(\frac{C_3}{w}\right)^{\alpha}\tau(-w)>w\tau(0)$,\\
     (b) $C_2> \beta^{1/2}+w$,\\
      (c) $C_1\Phi(-w)>1$,\\ 
   (d) $\tau(C_3x-w)-x\tau(0)>0$\\
   for $x\in (0,\frac{w}{C_3})$, where $C_3=C_2-\beta^{1/2}$. 
   Running the BO-EI algorithm with GP prior $(0,k(\xbm,\xbm'))$ leads to the convergence rate 
      \begin{equation} \label{eqn:EI-convg-star-1}
  \centering
  \begin{aligned}
      r_t  \leq C_1 (2M+2c_\sigma\sigma)\frac{3}{t}+\max\{C_1\beta^{1/2}+C_2,0.4+2\beta^{1/2}\} \sigma_{t_k}^{\alpha}(\xbm_{t_k}), 
   \end{aligned}
  \end{equation} 
  for some $t_k\in [\frac{t}{3}-1,t]$, 
  with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-(\frac{1}{2})^{t/3}-2\Phi(-c_{\sigma})-\delta$.
\end{theorem}
\begin{proof}
  First, we note that the choice of $\beta$ is larger than the values required in Lemma~\ref{lem:IEIbound}, Lemma~\ref{lem:fmu}, and Lemma~\ref{lem:fmu-alpha} to achieve a probability $\geq 1-\delta/3$, \textit{i.e.},~\eqref{eqn:IEI-bound-1} and~\eqref{eqn:fmu-a-1} stand with probability $\geq 1-\delta/3$ each. 
  Similar to Theorem~\ref{theorem:EI-convergence-1}, we know that with probability $\geq 1-2\Phi(-c_{\sigma})$,
  \begin{equation} \label{eqn:EI-convg-star-pf-1}
  \centering
  \begin{aligned}
        \sum_{t=0}^{T-1}  y^+_{t}-y^+_{t+1} \leq y^+_0 - y_T^+ \leq 2 M +2c_{\sigma}\sigma. 
  \end{aligned}
  \end{equation}
  Therefore, $y^+_{t}-y^+_{t+1} \geq \frac{2M +2c_{\sigma}\sigma}{k}$ at most $k$ times for any $k\in \Nbb$.
  Choose $k=[t/2]$, where $[x]$ is the largest integer smaller than $x$ so that $2k\leq t\leq 2(k+1)$.
  Then, there exists $k\leq t_k\leq 2k$ where $y^+_{t_k}-y^+_{t_k+1} < \frac{2M +2c_{\sigma}\sigma}{k}$. 
  We first consider the noiseless case $\sigma=0$.   

  From Lemma~\ref{lem:IEIbound}, with probability $\geq 1-\delta/3$,
  \begin{equation} \label{eqn:EI-convg-star-pf-2}
  \centering
  \begin{aligned}
          r_t =& y^+_{t}-f(\xbm^*)\leq y^+_{t_k}-f(\xbm^*)\leq I_{t_k}(\xbm^*)\\
               \leq& EI_{t_k}(\xbm^*,\alpha) + \beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm^*)
               \leq EI_{t_k}(\xbm_{t_k},\alpha) + \beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm^*)\\
                =& (y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\phi(z_{t_k}(\xbm_{t_k+1},\alpha))  + \beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm^*).\\
            \leq& (y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+0.4\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}) + \beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm^*),
   \end{aligned}
  \end{equation}
   where the last inequality uses $\phi(\cdot)<0.4$ from Lemma~\ref{lem:phi}.
    From Lemma~\ref{lem:fmu}, with probability $1-\delta/3$, 
   \begin{equation} \label{eqn:EI-convg-star-pf-5}
  \centering
  \begin{aligned}
          y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}) =& y^+_{t_k}-f(\xbm_{t_k+1})+f(\xbm_{t_k+1})-\mu_{t_k}(\xbm_{t_k+1}) \\
          \leq& y^+_{t_k}-y^+_{t_k+1}+\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1})\leq \frac{2M}{k} +\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}).
    \end{aligned}
  \end{equation}
  Applying~\eqref{eqn:EI-convg-star-pf-5} to~\eqref{eqn:EI-convg-star-pf-2}, we have with probability $\geq 1-2/3\delta$, 
  \begin{equation} \label{eqn:EI-convg-star-pf-6}
  \centering
  \begin{aligned}
          r_t  \leq& \frac{2M}{k}+0.4\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})+\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}) + \beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm^*).\\
  \end{aligned}
  \end{equation}

  Since $\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1})\to 0$ as $t\to\infty$, to obtain convergence of $r_t$, from~\eqref{eqn:EI-convg-star-pf-6}, we need to consider the convergence behavior of $\sigma_{t_k}(\xbm^*)$ with respect to $\sigma_{t_k}(\xbm_{t_k+1})$.
   By the definition of $\xbm_{t_k+1}$, it generates the largest $EI_{t_k}$, \textit{i.e.},
   \begin{equation} \label{eqn:EI-convg-star-pf-7}
  \centering
  \begin{aligned}
        EI_{t_k}(\xbm_{t_k+1},\alpha) > EI_{t_k}(\xbm^*,\alpha).
    \end{aligned}
  \end{equation}
   From the proof of Lemma~\ref{lem:fmu-alpha}, we know for $w>0$, 
   \begin{equation} \label{eqn:EI-convg-star-pf-8}
   \centering
   \begin{aligned}
       P\{ f(\xbm^*)-\mu_{t_k}(\xbm^*) > -\sigma_{t_k}(\xbm^*) w\}\geq 1-\frac{1}{2}e^{-w^2/2}=1-\sqrt{\frac{\pi}{2}}\phi(w).
    \end{aligned}
   \end{equation} 
   Then, with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)$, $f(\xbm^*)-\mu_{t_k}(\xbm^*) > -w\sigma_{t_k}(\xbm^*)$. Using $\delta/3$ at $t_k$ in Lemma~\ref{lem:fmu}, with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta/3$,
   \begin{equation} \label{eqn:EI-convg-star-pf-9}
   \centering
   \begin{aligned}
      &y^+_{t_k}-\mu_{t_k}(\xbm^*)>y^+_{t_k}-f(\xbm^*)- w\sigma_{t_k}(\xbm^*) = y^+_{t_k}-f(\xbm_{t_k+1})+f(\xbm_{t_k+1})-f(\xbm^*)- w\sigma_{t_k}(\xbm^*)\\
          =& y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1})+\mu_{t_k}(\xbm_{t_k+1})-f(\xbm_{t_k+1})+f(\xbm_{t_k+1})-f(\xbm^*)- w\sigma_{t_k}(\xbm^*)\\
           \geq& y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}) +f(\xbm_{t_k+1})-f(\xbm^*)- w\sigma_{t_k}(\xbm^*)-\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}).
    \end{aligned}
   \end{equation}
   With $\sigma=0$, $y_{t}=f(\xbm_{t})$ for  $\forall t\in \Nbb$. 
   We consider two scenarios regarding the term $f(\xbm_{t_k+1})-f(\xbm^*)$ in~\eqref{eqn:EI-convg-star-pf-9}.
   
   \textbf{Scenario A.} Suppose first that $f(\xbm_{t_k+1})-f(\xbm^*)$ reduces to $0$ at a fast enough rate to satisfy
   \begin{equation} \label{eqn:EI-convg-star-pf-9.5}
   \centering
   \begin{aligned}
      f(\xbm_{t_k+1})-f(\xbm^*) \leq C_1\max\{y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}),0\}+C_2 \sigma_{t_k}(\xbm_{t_k+1}),
    \end{aligned}
   \end{equation}
   where $C_1$ and $C_2$ are two constants in the statement of the theorem. 
    Then, from~\eqref{eqn:EI-convg-star-pf-5} and~\eqref{eqn:EI-convg-star-pf-9.5}, we have with probability $\geq 1-\delta/3$, 
   \begin{equation} \label{eqn:EI-convg-star-pf-10}
   \centering
   \begin{aligned}
         r_t= y^+_{t}-f(\xbm^*) \leq& y^+_{t_k+1}-f(\xbm^*) \leq f(\xbm_{t_k+1})-f(\xbm^*) \leq C_1 \frac{2M}{k}+(C_1\beta^{1/2}+C_2)\sigma_{t_k}(\xbm_{t_k+1}),
    \end{aligned}
   \end{equation}
   which then proves the theorem.
   
  \textbf{Scenario B.} Next, we analyze the second scenario where
   \begin{equation} \label{eqn:EI-convg-star-pf-11}
   \centering
   \begin{aligned}
     f(\xbm_{t_k+1})-f(\xbm^*) >  C_1\max\{y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}),0\}+C_2\sigma_{t_k}(\xbm_{t_k+1}). 
    \end{aligned}
   \end{equation}
    We make the claim that in this scenario, $\sigma_{t_k}(\xbm^*)\leq \sigma_{t_k}(\xbm_{t_k+1})$  with a high probability under the conditions for the constants in the statement of the theorem. We prove by contradiction. Suppose on the contrary,   
  \begin{equation} \label{eqn:EI-convg-star-pf-premise}
  \centering
  \begin{aligned}
     \sigma_{t_k}(\xbm_{t_k+1})     < \sigma_{t_k}(\xbm^*)\leq 1,
  \end{aligned}
  \end{equation}
   with probability $1-\delta_{\sigma}$.
   Since $ y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1})$ is bounded by $\sigma_{t_k}(\xbm_{t_k+1})$ by the choice of $t_k$, we claim that by choosing finite $C_1$ and $C_2$ large enough to satisfy conditions (a)-(d),~\eqref{eqn:EI-convg-star-pf-premise} contradicts~\eqref{eqn:EI-convg-star-pf-7}, and thus under the second scenario~\eqref{eqn:EI-convg-star-pf-11}, we have $\sigma_{t_k}(\xbm_{t_k+1}) \geq\sigma_{t_k}(\xbm^*)$ with a high probability. 
   While our conditions $(a)-(d)$ are given in constants $C_1,C_2,w$, a simple example that would suffice is $C_1=C_3=100$ and $w=2$, with the probability $1-\sqrt{\frac{\pi}{2}}\phi(w)=0.932$ at a high level. More discussion on the constants are given in Remark~\ref{}.

   To proceed, we use the notation of exploitation and exploration for EI~\eqref{eqn:EI-ab}. Let $a_{t_k}=y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1})$ and $b_{t_k}= \sigma_{t_k}^{\alpha}(\xbm_{t_k+1})$.
   Based on~\eqref{eqn:EI-convg-star-pf-9} and~\eqref{eqn:EI-convg-star-pf-premise}, at $\xbm^*$,  let $b^*_{t_k}=\sigma_{t_k}^{\alpha}(\xbm^*)$ and  
   \begin{equation} \label{eqn:EI-convg-star-pf-12}
   \centering
   \begin{aligned}
          a^*_{t_k} &= y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1})+C_1\max\{y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}),0\}+C_2\sigma_{t_k}(\xbm_{t_k+1})\\
  &-w \sigma_{t_k}(\xbm^*)-\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}) =a_{t_k}+C_1\max\{a_{t_k},0\}-w(b^*_{t_k})^{\frac{1}{\alpha}}+(C_2-\beta^{1/2})b_{t_k}^{\frac{1}{\alpha}}. 
    \end{aligned}
   \end{equation}
   Thus, $b^*_{t_k}>b_{t_k}$ with probability $\geq 1-\delta_{\sigma}$ by~\eqref{eqn:EI-convg-star-pf-premise}.
   Moreover, using~\eqref{eqn:EI-convg-star-pf-9},~\eqref{eqn:EI-convg-star-pf-11}, and~\eqref{eqn:EI-convg-star-pf-12}
   \begin{equation} \label{eqn:EI-convg-star-pf-12.5}
   \centering
   \begin{aligned}
      y^+_{t_k}-\mu_{t_k}(\xbm^*)\geq a^*_{t_k},
    \end{aligned}
   \end{equation}
with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta/3$.
   Since EI is monotonically increasing with respect to both $a_{t_k}$ and $b_{t_k}$ by Lemma~\ref{lem:EI-ms}, from~\eqref{eqn:EI-convg-star-pf-premise},~\eqref{eqn:EI-convg-star-pf-12.5} and union bound, we have  
   \begin{equation} \label{eqn:EI-convg-star-pf-13}
   \centering
   \begin{aligned}
          EI_{t_k}(\xbm^*,\alpha) =EI(y^+_{t_k}-\mu_{t_k}(\xbm^*),\sigma_{t_k}^{\alpha}(\xbm^*)) \geq EI(a^*_{t_k},b^*_{t_k}),
    \end{aligned}
   \end{equation}
  with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta/3-\delta_{\sigma}$.
   Denote $C_3=C_2-\beta^{1/2}$. We consider two cases regarding $b_{t_k}^*$ and~\eqref{eqn:EI-convg-star-pf-12}.
   
   \textbf{Case 1.} If 
   \begin{equation} \label{eqn:EI-convg-star-pf-13.2}
   \centering
   \begin{aligned}
          b^*_{t_k} < \left[\frac{C_1}{w}\max\{a_{t_k},0\}+\frac{C_3}{w}b_{t_k}^{\frac{1}{\alpha}}\right]^{\alpha},
    \end{aligned}
   \end{equation}
   then by~\eqref{eqn:EI-convg-star-pf-12},
   \begin{equation} \label{eqn:EI-convg-star-pf-13.3}
   \centering
   \begin{aligned}
      a^*_{t_k} > a_{t_k}, \ \text{and} \ EI(a^*_{t_k},b^*_{t_k}) > EI(a_{t_k},b_{t_k})=EI_{t_k}(\xbm_{t_k+1},\alpha).
    \end{aligned}
   \end{equation}
   
   \textbf{Case 2.} Next we consider the case where 
   \begin{equation} \label{eqn:EI-convg-star-pf-13.5}
   \centering
   \begin{aligned}
          b^*_{t_k} \geq \left[\frac{C_1}{w}\max\{a_{t_k},0\}+\frac{C_3}{w}b_{t_k}^{\frac{1}{\alpha}}\right]^{\alpha}\geq \left(\frac{C_3}{w}\right)^{\alpha} b_{t_k}.
    \end{aligned}
   \end{equation} 
   Moreover, from~\eqref{eqn:EI-convg-star-pf-premise}, $\frac{b_{t_k^*}}{b_{t_k}}>1$. Without losing generality, we can assume $\frac{C_3}{w}>1$. 
   (In general, to satisfy conditions (a)-(c), $\frac{C_3}{w}> 1$ is implied.)
   We further distinguish between two cases based on the sign of $a_{t_k}$.

   \textbf{Case 2.1.} 
   First, if $a_{t_k}<0$ and thus $z_{t_k}=a_{t_k}/b_{t_k}<0$, we can write using~\eqref{eqn:EI-convg-star-pf-13.5}, 
    \begin{equation} \label{eqn:EI-convg-star-pf-14}
   \centering
   \begin{aligned}
            EI(a^*_{t_k},b^*_{t_k}) =& EI(a_{t_k}+C_3b_{t_k}^{\frac{1}{\alpha}}-w(b^*_{t_k})^{\frac{1}{\alpha}},b^*_{t_k}) = b^*_{t_k} \tau\left(\frac{a_{t_k}+C_3b_{t_k}^{\frac{1}{\alpha}}-w(b^*_{t_k})^{\frac{1}{\alpha}}}{b^*_{t_k}}\right) \\
             \geq& \left(\frac{C_3}{w}\right)^{\alpha} b_{t_k} \tau\left((z_{t_k}+C_3b_{t_k}^{\frac{1-\alpha}{\alpha}})\frac{b_{t_k}}{b^*_{t_k}}-w(b^*_{t_k})^{\frac{1-\alpha}{\alpha}}\right).
    \end{aligned}
   \end{equation}

   \textbf{Case 2.1.1.} 
  If $z_{t_k}>-C_3b_{t_k}^{\frac{1-\alpha}{\alpha}}$,
    \begin{equation} \label{eqn:EI-convg-star-pf-14.5}
   \centering
   \begin{aligned}
(z_{t_k}+C_3b_{t_k}^{\frac{1-\alpha}{\alpha}})\frac{b_{t_k}}{b^*_{t_k}}-w(b^*_{t_k})^{\frac{1-\alpha}{\alpha}}
     > -w(b^*_{t_k})^{\frac{1-\alpha}{\alpha}}>-w,
    \end{aligned}
   \end{equation}
  where the last inequality uses $b^*_{t_k}\in (0,1]$ and $\alpha\in (0,1]$.
  From~\eqref{eqn:EI-convg-star-pf-14},~\eqref{eqn:EI-convg-star-pf-14.5}, and condition (a) $(\frac{C_3}{w})^{\alpha}\tau(-w)>\tau(0)$, \textit{e.g.}, $50\tau(-2)>\tau(0)$, we have by the monotonicity of $\tau(\cdot)$ (Lemma~\ref{lem:phi}) 
    \begin{equation} \label{eqn:EI-convg-star-pf-15}
   \centering
   \begin{aligned}
            EI(a^*_{t_k},b^*_{t_k})  >& \left(\frac{C_3}{w}\right)^{\alpha} b_{t_k} \tau\left(-w\right)> b_{t_k}\tau(0) \geq b_{t_k}\tau(z_{t_k}) \geq EI(a_{t_k},b_{t_k}).
    \end{aligned}
   \end{equation}
  
   \textbf{Case 2.1.2.} 
  If $z_{t_k}<-C_3b_{t_k}^{\frac{1-\alpha}{\alpha}}$, then by~\eqref{eqn:EI-convg-star-pf-13.5},
  $\frac{b_{t_k}}{b^*_{t_k}}\leq (\frac{w}{C_3})^{\alpha}<1$.
    Using the monotonicity of $\tau(\cdot)$,~\eqref{eqn:EI-convg-star-pf-14} implies  
    \begin{equation} \label{eqn:EI-convg-star-pf-16}
   \centering
   \begin{aligned}
            EI(a^*_{t_k},b^*_{t_k}) 
             \geq& \left(\frac{C_3}{w}\right)^{\alpha} b_{t_k} \tau\left(\left(\frac{w}{C_3}\right)^{\alpha}(z_{t_k}+C_3b_{t_k}^{\frac{1-\alpha}{\alpha}})-w \right) \\
             \geq& \left(\frac{C_3}{w}\right)^{\alpha} b_{t_k} \tau\left(\left(\frac{w}{C_3}\right)^{\alpha}z_{t_k}-w \right).
    \end{aligned}
   \end{equation}
   Denote $(\frac{w}{C_3})^{\alpha}=\rho<1$. Then,~\eqref{eqn:EI-convg-star-pf-16} becomes 
    \begin{equation} \label{eqn:EI-convg-star-pf-16.2}
   \centering
   \begin{aligned}
            EI(a^*_{t_k},b^*_{t_k}) 
             \geq& \frac{1}{\rho} b_{t_k} \tau\left( \rho z_{t_k}-w \right).
    \end{aligned}
   \end{equation}
   Recall $z_{t_k}<0$. By~\eqref{eqn:EI-convg-star-pf-16.2}, we have  
    \begin{equation} \label{eqn:EI-convg-star-pf-16.3}
   \centering
   \begin{aligned}
    EI(a_{t_k}^*,b_{t_k}^*)-EI(a_{t_k},b_{t_k}) = b_{t_k} \left[ \frac{1}{\rho} \tau\left( \rho z_{t_k}-w \right) - \tau(z_{t_k})\right].
    \end{aligned}
   \end{equation}

   \textbf{Case 2.1.2.1.}   
   If $\rho z_{t_k} -w>z_{t_k}$, \textit{i.e.}, $z_{t_k} \leq \frac{-w}{1-\rho}$, 
   by the monotonicity of $\tau$,
     \begin{equation} \label{eqn:EI-convg-star-pf-16.4}
   \centering
   \begin{aligned}
    EI(a_{t_k}^*,b_{t_k}^*)-EI(a_{t_k},b_{t_k}) = b_{t_k} \left[ \frac{1}{\rho} \tau\left( \rho z_{t_k}-w \right) - \tau(z_{t_k})\right]>0.
    \end{aligned}
   \end{equation}
   
   \textbf{Case 2.1.2.2.} 
   If  $z_{t_k} >\frac{-w}{1-\rho}$, we define function $\bar{\tau}$
    \begin{equation} \label{eqn:EI-convg-star-pf-16.5}
   \centering
   \begin{aligned}
     \bar{\tau}(x) =  \frac{1}{\rho} \tau\left( \rho x-w \right) - \tau(x), 
    \end{aligned}
   \end{equation}
  for $x>\frac{-w}{1-\rho}$. Taking the derivative of~\eqref{eqn:EI-convg-star-pf-16.5}, by Lemma~\ref{lem:tau}, we have 
    \begin{equation} \label{eqn:EI-convg-star-pf-16.7}
   \centering
   \begin{aligned}
     \frac{d\bar{\tau}}{d x} =  \frac{1}{\rho} \Phi\left( \rho x-w \right) \rho - \Phi(x) =  \Phi\left( \rho x-w \right) - \Phi(x) <0.
    \end{aligned}
   \end{equation}
  Therefore, for $0>z_{t_k}>\frac{-w}{1-\rho}$,  
    \begin{equation} \label{eqn:EI-convg-star-pf-16.8}
   \centering
   \begin{aligned}
     \bar{\tau}(z_{t_k}) \geq \bar{\tau}(0) = \frac{1}{\rho} \tau (-w) - \tau(0) = \left(\frac{C_3}{w}\right)^{\alpha} \tau (-w) - \tau(0)>0, 
    \end{aligned}
   \end{equation}
  given condition (a).
 Using~\eqref{eqn:EI-convg-star-pf-16.3} and~\eqref{eqn:EI-convg-star-pf-16.8},
    \begin{equation} \label{eqn:EI-convg-star-pf-16.9}
   \centering
   \begin{aligned}
    EI(a_{t_k}^*,b_{t_k}^*)-EI(a_{t_k},b_{t_k}) = b_{t_k}\bar{\tau}(z_{t_k}) >0.
    \end{aligned}
   \end{equation}
   Combining~\eqref{eqn:EI-convg-star-pf-16.4} and~\eqref{eqn:EI-convg-star-pf-16.9}, when $z_{t_k}<-C_3b_{t_k}^{\frac{1-\alpha}{\alpha}}$, $EI(a_{t_k}^*,b_{t_k}^*)> EI(a_{t_k},b_{t_k})$  (\textbf{Case 2.1.2}). 
   Further, combined with~\eqref{eqn:EI-convg-star-pf-15}, we have $EI(a^*_{t_k},b^*_{t_k})>EI(a_{t_k},b_{t_k})$ if $a_{t_k}<0$
 (\textbf{Case 2.1.}). 
    
   \textbf{Case 2.2.}
   In the second case, $a_{t_k}\geq 0$.  
   By definition~\eqref{eqn:EI-convg-star-pf-12}, 
     \begin{equation} \label{eqn:EI-convg-star-pf-17}
   \centering
   \begin{aligned}
            EI(a^*_{t_k},b^*_{t_k}) =& EI((C_1+1)a_{t_k}+C_3b_{t_k}^{\frac{1}{\alpha}}-w(b^*_{t_k})^{\frac{1}{\alpha}},b^*_{t_k}) 
              \geq b^*_{t_k} 
\tau\left((C_1 z_{t_k}+C_3b_{t_k}^{\frac{1-\alpha}{\alpha}}) \rho_{t_k} -w(b^*_{t_k})^{\frac{1-\alpha}{\alpha}}\right)\\
             =& b_{t_k} \frac{1}{\rho_{t_k}} \tau\left( C_1z_{t_k}\rho_{t_k}+ (C_3\rho_{t_k}^{\frac{1}{\alpha}}-w)(b^*_{t_k})^{\frac{1-\alpha}{\alpha}}\right),
    \end{aligned}
   \end{equation}
   where $\rho_{t_k}=\frac{b_{t_k}}{b^*_{t_k}}$
    By~\eqref{eqn:EI-convg-star-pf-13.5} and $a_{t_k}\geq 0$,
     \begin{equation} \label{eqn:EI-convg-star-pf-17.2}
   \centering
   \begin{aligned}
      \rho_{t_k}\leq \left( \frac{w}{C_3}-\frac{C_1}{C_3} \frac{a_{t_k}}{(b_{t_k}^*)^{\frac{1}{\alpha}}}\right)^{\alpha}\leq \left( \frac{w}{C_3}-\frac{C_1}{C_3} a_{t_k}\right)^{\alpha}\leq \left( \frac{w}{C_3}\right)^{\alpha}.
    \end{aligned}
   \end{equation}
  Thus,
     \begin{equation} \label{eqn:EI-convg-star-pf-17.3}
   \centering
   \begin{aligned}
       C_3\rho_{t_k}^{\frac{1}{\alpha}}-w \leq 0.
    \end{aligned}
   \end{equation}
  Applying~\eqref{eqn:EI-convg-star-pf-17.3} and $b_{t_k}^*\in (0,1]$ to~\eqref{eqn:EI-convg-star-pf-17}, we have
   \begin{equation} \label{eqn:EI-convg-star-pf-17.4}
   \centering
   \begin{aligned}
            EI(a^*_{t_k},b^*_{t_k}) 
             \geq b_{t_k} \frac{1}{\rho_{t_k}} \tau\left( C_1z_{t_k}\rho_{t_k}+ C_3\rho_{t_k}^{\frac{1}{\alpha}}-w\right).
    \end{aligned}
   \end{equation}
  Define function $\tilde{\tau}$ as 
     \begin{equation} \label{eqn:EI-convg-star-pf-17.5}
   \centering
   \begin{aligned}
    \tilde{\tau}(\rho,z) = 
\frac{1}{\rho} \tau\left( C_1 z\rho+ C_3\rho^{\frac{1}{\alpha}}-w\right),
    \end{aligned}
   \end{equation}
   for $\rho\in (0,(\frac{w}{C_3})^{\alpha}), z\geq 0$.
   From~\eqref{eqn:EI-convg-star-pf-17.4}, $EI(a^*_{t_k},b^*_{t_k})\geq b_{t_k}\tilde{\tau}(\rho_{t_k},z_{t_k})$.
    We now compare $ \tilde{\tau}(\rho_{t_k},z_{t_k})$ and $\tau(z_{t_k})$. For $\forall \rho_{t_k}\in (0,(\frac{w}{C_3})^{\alpha})$, condition $(c)$ $C_1\Phi(-w)\geq 1$ and Lemma~\ref{lem:tau} lead to the derivative 
     \begin{equation} \label{eqn:EI-convg-star-pf-18}
   \centering
   \begin{aligned}
         \frac{\partial \tilde{\tau}}{\partial z}|_{(\rho_{t_k},z_{t_k}) } = C_1 \Phi\left(C_1z_{t_k}\rho_{t_k}+C_3\rho_{t_k}^{\frac{1}{\alpha}}-w\right)>C_1\Phi(-w)\geq \Phi(z_{t_k})=\frac{d \tau}{d z}|_{z_{t_k}}.
    \end{aligned}
   \end{equation}
   Therefore, both $\tilde{\tau}(\cdot,\cdot)$ and $\tau(\cdot)$ are monotonically increasing with $z_{t_k}$ and $\tilde{\tau}$ always has a larger positive derivative. For any $\rho_{t_k}$, this leads to
     \begin{equation} \label{eqn:EI-convg-star-pf-19}
   \centering
   \begin{aligned}
      \tilde{\tau}(\rho_{t_k},z_{t_k}) - \tau(z_{t_k}) \geq \tilde{\tau}(\rho_{t_k},0)-\tau(0)=\frac{1}{\rho_{t_k}}\tau\left(C_3\rho_{t_k}^{\frac{1}{\alpha}}-w \right)-\tau(0).
    \end{aligned}
    \end{equation}
  The right-hand side of the inequality in~\eqref{eqn:EI-convg-star-pf-19} is a complex function of $\rho_{t_k}$. For example, for $C_3=100$, $w=2$ and $\alpha=1$, it obtains a minimum value of $5.4$, see figure~\ref{}. 
  
  Given condition $(d)$ $\frac{1}{x}\tau(C_3x^{\frac{1}{\alpha}}-w)-\tau(0)>0$ for $x\in(0,(\frac{w}{C_3})^{\alpha})$, by~\eqref{eqn:EI-convg-star-pf-17.4} and~\eqref{eqn:EI-convg-star-pf-19}, we have 
     \begin{equation} \label{eqn:EI-convg-star-pf-20}
   \centering
   \begin{aligned}
            EI(a^*_{t_k},b^*_{t_k}) \geq b_{t_k} \tilde{\tau}(\rho_{t_k},z_{t_k})> b_{t_k}\tau(z_{t_k}) = EI(a_{t_k},b_{t_k}).
    \end{aligned}
   \end{equation}

    To summarize, under the \textbf{Scenario B Case 2}, for all cases given~\eqref{eqn:EI-convg-star-pf-13.5}, 
   $EI(a_{t_k}^*,b_{t_k}^*)>EI(a_{t_k},b_{t_k})$.
   Combined with~\eqref{eqn:EI-convg-star-pf-13.2}, under \textbf{Scenario B}, $EI(a_{t_k}^*,b_{t_k}^*)>EI(a_{t_k},b_{t_k})$.

   From~\eqref{eqn:EI-convg-star-pf-13}, with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta/3-\delta_{\sigma}$, $EI(\xbm^*,\alpha)>EI(\xbm_{t_k},\alpha)$. However, this is a contradiction of~\eqref{eqn:EI-convg-star-pf-7}, a sure event.
   Therefore, we have   
 \begin{equation} \label{eqn:EI-convg-star-pf-20.5}
   \centering
   \begin{aligned}
   1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta/3-\delta_{\sigma}\leq 0.
    \end{aligned}
   \end{equation}
   That is, $\delta_{\sigma}\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta/3$. From~\eqref{eqn:EI-convg-star-pf-premise},
 \begin{equation} \label{eqn:EI-convg-star-pf-21}
   \centering
   \begin{aligned}
           \sigma_{t_k}(\xbm_{t_k+1})\geq \sigma_{t_k}(\xbm^*),
    \end{aligned}
   \end{equation}
   with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta/3$.
   Under \textbf{Scenario B}, by~\eqref{eqn:EI-convg-star-pf-21} and~\eqref{eqn:EI-convg-star-pf-6}, with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta$,  
     \begin{equation} \label{eqn:EI-convg-star-pf-22}
   \centering
   \begin{aligned}
       r_t \leq \frac{2M}{k} + (0.4+\beta^{1/2})\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})+\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}).
     \end{aligned}
   \end{equation}
    Combining \textbf{Scenario A}~\eqref{eqn:EI-convg-star-pf-10} and \textbf{Scenario B}~\eqref{eqn:EI-convg-star-pf-21}, $r_t$ must be decreasing with the same rate as $\sigma_{t_k}(\xbm_{t_k+1})$ with probability $\geq 1-\sqrt{\frac{\pi}{2}}\phi(w)-\delta$, provided that $\frac{1}{t}=o(\sigma_{t_k}(\xbm_{t_k+1}))$.
  

   Finally, we consider the noisy case using similar technique as in Theorem~\ref{theorem:EI-convergence-1}. Since majority of the proof is the same as the noiseless case, we only provide a sketch of proof here. Given a sequence of iterates $\xbm_i$  of size $k\in \Nbb$ where $i\in A_k$, \textit{i.e.}, $|A_k|=k$, the probability of $f(\xbm_i) < y_i = f(\xbm_i)+\epsilon(\xbm_i)$ for $\forall i\in A_k$ is $(\frac{1}{2})^k$.
  Let $k=[t/3]$ so that $3k\leq t\leq 3(k+1)$. There exists $k \leq t_k \leq 3k$ so that $y_{t_k}^+-y_{t_k+1}^+<\frac{2M_f+2c_{\sigma}\sigma}{k}$ and $f(\xbm_{t_k+1})\geq y_{t_k+1}\geq y_{t_k+1}^+$ with probability $\geq 1-(\frac{1}{2})^k$.
  Under the \textbf{Scenario A}~\eqref{eqn:EI-convg-star-pf-10},
  \begin{equation} \label{eqn:EI-convg-star-pf-23}
  \centering
  \begin{aligned}
     r_t \leq& C_1  \frac{2M+2c_{\sigma}\sigma}{k}+(C_1\beta^{1/2}+C_2)\sigma_{t_k}(\xbm_{t_k+1}),
  \end{aligned}
  \end{equation}
  with probability $\geq 1-(\frac{1}{2})^k-\delta/3-2\Phi(-c_{\sigma})$, 
  Similar to~\eqref{eqn:EI-convg-star-pf-22}, under \textbf{Scenario B}, 
  with probability $\geq 1-(\frac{1}{2})^k-\sqrt{\frac{\pi}{2}}\phi(w)-\delta-2\Phi(-c_{\sigma})$, 
  \begin{equation} \label{eqn:EI-convg-star-pf-24}
  \centering
  \begin{aligned}
         r_t  \leq& \frac{2M+2c_{\sigma}\sigma}{k}+(0.4+ \beta^{1/2})\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}) + \beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}).\\
  \end{aligned}
  \end{equation}
  Following the same analysis for the noiseless case, with probability $\geq 1-(\frac{1}{2})^k-\sqrt{\frac{\pi}{2}}\phi(w)-\delta-2\Phi(-c_{\sigma})$, $r_t$ satisfies~\eqref{eqn:EI-convg-star-1}.
\end{proof}
\begin{remark}
   We note that the analysis is not applicable to cumulative regret bounds since the probability of union bounds on $\beta$ would not be summable. 
 A natural question is how large should $w$ be. The probability $\sqrt{\frac{\pi}{2}}\phi(w)$ reduces exponentially with $w$. It is possible to ask for $w\to\infty$. However, to maintain convergence, we need $C_2\to\infty$ much faster.

All under the assumption that $\sigma_{t}(\xbm)$ can only be upper bounded by $1$. This restricts the conditions on the constants.
If we allow a lower bound, \textit{e.g.} $\sigma_t(\xbm^*)\leq \sigma_t(\xbm_{t+1})$, it is possible better bounds can be achieved. 
The choice of $k$ is arbitrary. It can even be $\log(t)$!
 \textbf{Add} contour plots for $\tilde{\tau}$ and $\bar{\tau}$ and other combinations of $C_1$, $C_2$, and $w$.
\end{remark}
\subsection{Discussion of parameters}\label{se:alpha}
It is complicated for $\alpha$, not monotonic. Probably will just leave it here.



==> Sections/EI.tex <==
\section{Cumulative regret of EI}\label{se:ei-regret}
In this section, we consider the cumulative regret of BO-EI under Assumptions~\ref{assp:rkhs} and~\ref{assp:constraint}. 
Since the instantaneous regret $r_t$ measures the loss in reward function, we propose a novel definition based on the structure of EI as 
 \begin{equation} \label{eqn:cumu-error}
 \centering
  \begin{aligned}
       r_t = I_{t-1}(\xbm^*) - I_{t-1}(\xbm_{t}) = \max\{y^+_{t-1}-f(\xbm^*),0\}-\max\{y^+_{t-1}-f(\xbm_{t}),0\}\geq 0.
  \end{aligned}
\end{equation}
   We note that $r_t$ in~\eqref{eqn:cumu-error} is non-negative since $f(\xbm^*)\leq f(\xbm_{t+1})$.
   The main difference between~\eqref{eqn:cumu-error} and~\eqref{eqn:rt-1} is that instead of $f$, we use the improvement function $I_t$.
   Given that EI is constructed upon the improvement function, $I_t$ is a reasonable measure of reward.
Further, the observation $y^+_t$ and improvement function $I_t$  are fully incorporated in the BO-EI algorithm to determine the next best sample.
  Therefore, the adoption of $I_t$ is a natural extension of the algorithm itself. 
  From the theoretical perspective,~\eqref{eqn:cumu-error} allows us to overcome the difficulty in providing a lower bound for $y_t^+-f(\xbm_{t+1})$ when $y_t^+-f(\xbm_{t+1})<0$, as its contribution to $r_t$ measures $0$. 
  This is an important step that previous papers dealt with by requiring additional modification of EI. 
  For example, in~\cite{nguyen17a}, the authors used a stopping criterion to achieve a lower bound. Others have resorted to modification of the BO-EI algorithm with new algorithmic parameters~\cite{tran2022regret}. 


We note that the analysis framework in this section bears similarity to that in section~\ref{se:regret} in that we assume first a discrete $C$ and then extends to be a compact set, as in~\cite{srinivas2009gaussian}. 
Further, the proofs and conclusions can be easily extended to GP prior assumption of the objective~\cite{} and Gaussian noise.
The following lemma is a direct result from~\cite{}.
\begin{lemma}\label{lem:EI}
 $EI_t(\xbm)$ satisfies the following properties
\begin{equation} \label{eqn:EI-property-1}
 \centering
  \begin{aligned}
    EI_t(\xbm) \geq 0, EI_t(\xbm) \geq y^+_{t}- \mu_{t}(\xbm).
  \end{aligned}
\end{equation}
Moreover, 
\begin{equation} \label{eqn:EI-property-2}
 \centering
  \begin{aligned}
   z_{t}(\xbm) \sigma_{t}(\xbm)\leq EI_{t}(\xbm) < \begin{cases}  \phi(z_{t}(\xbm))\sigma_{t}(\xbm), \ &z_{t}(\xbm)<0\\
             [z_{t}(\xbm) +\phi(z_{t}(\xbm))]\sigma_{t}(\xbm), \ &z_{t}(\xbm)\geq 0.
      \end{cases}
  \end{aligned}
\end{equation}

\end{lemma}
We quantify $I_t(\xbm)-EI_t(\xbm)$ in the next two lemmas.
\begin{lemma}\label{lem:fandnu}
For $\forall \xbm\in C$ and $w>0$,   
\begin{equation} \label{eqn:fandmu-1}
 \centering
  \begin{aligned}
    I_t(\xbm) - EI_t(\xbm)  < \begin{cases} \sigma_t(\xbm) w, \  &y^+_t- f(\xbm)\leq 0\\
                     -f(\xbm) +\mu_t(\xbm),  \ & y^+_t-f(\xbm)>0.
         \end{cases}
  \end{aligned} 
\end{equation}
\end{lemma}
\begin{proof}
      If $y^+_t-f(\xbm)\leq 0$, we have by Lemma~\ref{lem:EI}, 
\begin{equation} \label{eqn:fandmu-pf-1}
 \centering
  \begin{aligned}
     I_t(\xbm)-EI_t(\xbm) =  - EI_t(\xbm)  < 0< \sigma_t(\xbm) w. 
  \end{aligned}
\end{equation}
For $y^+_t- f(\xbm)>0$, we can write via Lemma~\ref{lem:EI}, 
\begin{equation} \label{eqn:fandmu-pf-2}
 \centering
  \begin{aligned}
   I_t(\xbm)-EI_t(\xbm) = y^+_t- f(\xbm) - EI_t(\xbm)\leq  y^+_t-f(\xbm)-y^+_t+\mu_t(\xbm)  < -f(\xbm)+\mu_t(\xbm). 
  \end{aligned}
\end{equation}
\end{proof}

\begin{lemma}\label{lem:fnu-lower}
Let $w>1$. For $\forall \xbm\in C$, if $f(\xbm) - \mu_t(\xbm) < \sigma_t(\xbm) w$, then there exist $c_1,c_2>0$ such that 
\begin{equation} \label{eqn:fnu-lower-1}
 \centering
  \begin{aligned}
     I_t(\xbm) - EI_t(\xbm)   >  -\sigma_t(\xbm) w - \sigma_t(\xbm) c_1 e^{- c_2 w^2}, 
  \end{aligned}
\end{equation}
where $c_1,c_2>0$ are constant parameters.
\end{lemma}
\begin{proof}
    We consider two cases based on the sign of $EI_t(\xbm)-\sigma_t(\xbm)w$. 
First, $EI_t(\xbm)-\sigma_t(\xbm) w<0$. Given that $I_t(\xbm)\geq 0$, 
\begin{equation} \label{eqn:fnu-lower-pf-1}
 \centering
  \begin{aligned}
     I_t(\xbm) - EI_t(\xbm)   >  -\sigma_t(\xbm) w > -\sigma_t(\xbm) w- \sigma_t(\xbm) c_1 e^{- c_2 w^2},
  \end{aligned}
\end{equation}
  for any $c_1,c_2>0$.
  Second, $EI_t(\xbm)-\sigma_t(\xbm) w \geq 0$. We claim that $y^+_t-\mu_t(\xbm)\geq 0$ in this case. 
  Suppose on the contrary, $y^+_t-\mu_t(\xbm)<0$, then $z_t(\xbm)<0$. From~\eqref{eqn:EI-property-2}, 
\begin{equation} \label{eqn:fnu-lower-pf-2}
 \centering
  \begin{aligned}
      EI_t (\xbm)   \leq  \sigma_t(\xbm)\phi(z_t(\xbm))  < \sigma_t(\xbm) \phi(0) < \sigma_t(\xbm) w,
  \end{aligned}
\end{equation}
where the second inequality comes from the monotonicity of $\phi$ when $z_t(\xbm)\leq 0$ and the last inequality is due to $\phi(0)<1<w$. This contradicts the premise of the second case.
Therefore, $y^+_t-\mu_t(\xbm)\geq 0$ and  
\begin{equation} \label{eqn:fnu-lower-pf-3}
 \centering
  \begin{aligned}
     \frac{EI_t(\xbm)-y^+_t+\mu_t(\xbm)}{\sigma_t(\xbm)} =& z_t(\xbm) \Phi(z_t(\xbm)) + \phi(z_t(\xbm)) - z_t(\xbm) \\
          =& z_t(\xbm)[\Phi(z_t(\xbm))-1] + \phi(z_t(\xbm)) <\phi(z_t(\xbm)).
  \end{aligned}
\end{equation}
 Since $EI_t(\xbm)-\sigma_t(\xbm) w \geq 0$, 
\begin{equation} \label{eqn:fnu-lower-pf-4}
 \centering
  \begin{aligned}
    w\leq \frac{EI_t(\xbm)}{\sigma_t(\xbm)} = z_t(\xbm) \Phi(z_t(\xbm)) + \phi(z_t(\xbm))  < z_t(\xbm) + \phi(z_t(\xbm))\leq z_t(\xbm)+\phi(0).
  \end{aligned}
\end{equation}
  Using $w>1$ in~\eqref{eqn:fnu-lower-pf-4} , we know $z_t(\xbm) > 1-\phi(0)=0.601$. As $z_t(\xbm)$ increases, $\phi(z_t(\xbm))$ decreases. Thus, we have
\begin{equation} \label{eqn:fnu-lower-pf-5}
 \centering
  \begin{aligned}
    \frac{z_t(\xbm)}{\phi(z_t(\xbm))} > \frac{0.601}{\phi(0.601)} = 1.804.
  \end{aligned}
\end{equation}
  Applying~\eqref{eqn:fnu-lower-pf-5} to~\eqref{eqn:fnu-lower-pf-4}, we obtain
 \begin{equation} \label{eqn:fnu-lower-pf-6}
 \centering
  \begin{aligned}
     z_t(\xbm) > 0.643 w,  \ \phi(z_t(\xbm)) < \phi(0.643 w).
  \end{aligned}
\end{equation}
   Using~\eqref{eqn:fnu-lower-pf-6} in~\eqref{eqn:fnu-lower-pf-3}, we have
 \begin{equation} \label{eqn:fnu-lower-pf-7}
 \centering
  \begin{aligned}
     \frac{EI_t(\xbm)-y^+_t+\mu_t(\xbm)}{\sigma_t(\xbm)} < \phi(0.643 w) = \frac{1}{\sqrt{2\pi}}  e^{-\frac{1}{2}(0.643w)^2}< 0.4 e^{-0.21 w^2}.
  \end{aligned}
\end{equation}
Rearranging~\eqref{eqn:fnu-lower-pf-7} leads to 
 \begin{equation} \label{eqn:fnu-lower-pf-8}
 \centering
  \begin{aligned}
    -EI_t(\xbm) > -y^+_t+\mu_t(\xbm) - \sigma_t(\xbm) 0.4 e^{-0.21 w^2}.
  \end{aligned}
\end{equation}
  Therefore, from the condition of the lemma, 
 \begin{equation} \label{eqn:fnu-lower-pf-9}
 \centering
  \begin{aligned}
   I_t(\xbm) -EI_t(\xbm) > y^+_t-f(\xbm) -y^+_t+\mu_t(\xbm) - \sigma_t(\xbm) 0.4 e^{-0.21 w^2}>-\sigma_t(\xbm) w-\sigma_t(\xbm) 0.4 e^{-0.2 w^2}.
  \end{aligned}
\end{equation}
 Let $c_1\geq 0.4$ and $c_2\leq 0.21$ and the proof is complete.
\end{proof}
Using Lemma~\ref{lem:fandnu} and~\ref{lem:fnu-lower}, we have the following result. 
\begin{lemma}\label{lem:rkhs-bound-EI}
   Let $\delta\in(0,1)$. Let $\beta^{1/2}= c_3 (B+\frac{\sigma_{\epsilon}}{\sigma}\sqrt{2\log(1/\delta)})$ where $c_3 = 1.328$. Then, at given $\xbm \in C$ and $t\in\Nbb$ 
 \begin{equation} \label{eqn:rkhs-bound-2}
  \centering
  \begin{aligned}
     P\{|I_{t-1}(\xbm) - EI_{t-1}(\xbm)|\leq \beta^{1/2} \sigma_{t-1}(\xbm) \} \geq 1-\delta.
  \end{aligned}
\end{equation}
\end{lemma}
\begin{proof}
    Denote $\alpha^{1/2}= B+\frac{\sigma_{\epsilon}}{\sigma}\sqrt{2 \log(1/\delta)}$. 
 The choice of $\alpha$ satisfies Theorem~\ref{thm:rkhs-f-bound-finite}. Thus, $f(\xbm) - \mu_{t-1}(\xbm) \geq -\alpha^{1/2} \sigma_{t-1}(\xbm)$ with probability $\geq 1-\delta/2$.    
Using $w=\alpha^{1/2}$ in Lemma~\ref{lem:fandnu}, we have 
 \begin{equation} \label{eqn:rkhs-bound-pf-1}
  \centering
  \begin{aligned}
     I_t(\xbm) - EI_{t}(\xbm) \leq \alpha^{1/2} \sigma_{t}(\xbm) \leq c_3\alpha^{1/2} \sigma_t(\xbm) .
  \end{aligned}
\end{equation}
    Using $w=\alpha^{1/2}$ in  Lemma~\ref{lem:fnu-lower} leads to 
  \begin{equation} \label{eqn:rkhs-bound-pf-2}
  \centering
  \begin{aligned}
     I_t(\xbm) - EI_{t}(\xbm) \geq - \alpha^{1/2} \sigma_{t-1}(\xbm) - 0.4 e^{-0.21 \alpha } \sigma_{t-1}(\xbm) \geq -1.328 \alpha^{1/2} \sigma_{t-1}(\xbm) = -\beta^{1/2} \sigma_{t-1}(\xbm),
  \end{aligned}
\end{equation}
 with probability $\geq 1-\delta/2$.
 The second inequality in~\eqref{eqn:rkhs-bound-pf-2} is the result of an increasing $\alpha^{1/2}$ and an exponentially decreasing $e^{-0.21 \alpha }$ for $\alpha> 1$.
\end{proof}
Consider the discretization $\Cbb_t$. We can extend the results to $\forall \xbm\in, t\in\Rbb$.
\begin{lemma}\label{lem:EI-discret-bound-RKHS-2}
   Given $\delta\in(0,1)$, let $\beta_t^{1/2}= c_3(B+c_{\alpha}\sqrt{2\log(|\Cbb_t|\pi_t/\delta)})$ 
where $\sum_{t=1}^{\infty} \pi_t=1$, $c_{\alpha}=\frac{\sigma_{\alpha}}{\sigma}$, and $c_3=1.328$. 
   Then, for $\forall \xbm\in \Cbb_t$ and $\forall t\in\Nbb$,
      \begin{equation} \label{eqn:EI-discret-bound-RKHS-1}
  \centering
  \begin{aligned}
        |I_{t-1}(\xbm)-EI_{t-1}(\xbm)|\leq \beta_t^{1/2} \sigma_{t-1}(\xbm),
   \end{aligned}
  \end{equation} 
  with probability $\geq 1-\delta$.
\end{lemma}


\begin{lemma}\label{lem:EI-rkhs-bound-time-only}
   Let $\delta\in(0,1)$. Let $\beta^{1/2}= c_3(B+c_{\alpha}\sqrt{2\log(\pi_t/\delta)})$ 
where $\sum_{t=1}^{\infty} \pi_t=1$, $c_{\alpha}=\frac{\sigma_{\alpha}}{\sigma}$, and $c_3=1.328$. 
Then,  $\forall t\in\Nbb$ 
 \begin{equation} \label{eqn:EI-rkhs-bound-2}
  \centering
  \begin{aligned}
     P\{|I_{t-1}(\xbm_t) - EI_{t-1}(\xbm_t)|\leq \beta^{1/2}\sigma_{t-1}(\xbm_t) \} \geq 1-\delta.
  \end{aligned}
\end{equation}
\end{lemma}



\begin{lemma}\label{lem:EI-compact-rkhs-bound}
Given $\delta\in(0,1)$, let  $\beta_t^{1/2} = c_3 (B+c_{\alpha}\sqrt{2\log(\pi_t/\delta) + 2 d \log(c_t)}) $, 
where $\sum_{t=1}^{\infty} \pi_t=1$, $c_{\alpha}=\frac{\sigma_{\alpha}}{\sigma}$, $c_t 1+rt^2 L$, and $c_3=1.328$. 
   \begin{equation} \label{eqn:EI-compact-rkhs-bound-1}
  \centering
  \begin{aligned}
          |I_t(\xbm^*) - EI_{t}(\bar{\xbm}^*_t,\alpha)| \leq \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t) + \frac{1}{t^2},
  \end{aligned}
  \end{equation}
  for $\forall t\in\Nbb$.
\end{lemma}
\begin{proof}
  From Assumption~\ref{assp:lipschitz}, and Lemma~\ref{lem:lipschitz-cplus} in the Appendix, we know 
   \begin{equation} \label{eqn:EI-compact-rkhs-bound-pf-1}
  \centering
  \begin{aligned}
     | I_t(\xbm) - I_t(\xbm') | < L \norm{\xbm-\xbm'}.
  \end{aligned}
\end{equation}
   Applying the discretization $\Cbb_t$ and~\eqref{eqn:compactdisc-1} to~\eqref{eqn:EI-compact-rkhs-bound-pf-1}, for $\forall \xbm\in C$, we have 
   \begin{equation} \label{eqn:EI-compact-rkhs-bound-pf-2}
  \centering
  \begin{aligned}
     | I_t(\xbm_t) - I_t(\bar{\xbm}_t) | < L h_t = \frac{1}{t^2},
  \end{aligned}
\end{equation}
   where $L h_t  =\frac{1}{t^2}$ in~\eqref{eqn:ht-1} is used. 
   The cardinality of $\Cbb_t$ satisfies $|\Cbb_t| \leq (1+ r t^2 L)^d$. 
   The choice of $\beta_t$ in the condition of the lemma satisfies 
    the condition in Lemma~\ref{lem:EI-discret-bound-RKHS-2}. 
   Using~\eqref{eqn:EI-compact-rkhs-bound-pf-2} and Lemma~\ref{lem:EI-discret-bound-RKHS-2}, 
   \begin{equation} \label{eqn:EI-compact-rkhs-bound-pf-3}
  \centering
  \begin{aligned}
          |I_t(\xbm^*) - EI_{t}(\bar{\xbm}^*_t)| \leq& |I_t(\xbm^*) - I_t(\bar{\xbm}^*_t)| + |I_t(\bar{\xbm}^*_t) - EI_{t}(\bar{\xbm}^*_t)|\\ 
        \leq& \beta_t^{1/2} \sigma_{t}(\bar{\xbm}^*_t) + \frac{1}{t^2},
  \end{aligned}
\end{equation}
  with probability $\geq 1-\delta$.
\end{proof}

\begin{lemma}\label{lemma:EI-instregret-RKHS}
Given $\delta\in(0,1)$, let  $\beta_t^{1/2} = c_3 (B+c_{\alpha}\sqrt{2\log(2\pi_t/\delta) + 2 d \log( c_t)}) $, 
where $\sum_{t=1}^{\infty} \pi_t=1$, $c_{\alpha}=\frac{\sigma_{\alpha}}{\sigma}$, $c_t 1+rt^2 L$, and $c_3=1.328$. 
 Then, with probability $\geq 1-\delta$, 
      \begin{equation} \label{eqn:EI-instregret-RKHS-1}
  \centering
  \begin{aligned}
      r_t \leq&(\beta_t^{1/2}+0.4)\sigma_{t-1}(\xbm_{t})+ \beta^{1/2}_t\sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}. 
   \end{aligned}
  \end{equation} 
  with probability $\geq 1-\delta$.
\end{lemma}
\begin{proof}
    Notice that $\beta_t$ satisfies the conditions in both  Lemma~\ref{lem:EI-compact-rkhs-bound} and~\ref{lem:EI-bound-RKHS-t-only} with $\delta/2$. 
  If $y^+_{t}-f(\xbm_{t})\leq 0$, with probability $\geq 1-\delta$, 
   \begin{equation} \label{eqn:EI-instregret-RKHS-pf-1}
  \centering
  \begin{aligned}
          r_t  =& y^+_{t-1} - f(\xbm^*)  \leq I_{t-1}(\xbm^*) 
          \leq EI_{t-1}(\bar{\xbm}^*_t)  + \beta_t^{1/2} \sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq&  EI_{t-1}(\xbm_{t})  + \beta_t^{1/2} \sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          =& (y^+_{t-1}-\mu_{t-1}(\xbm_{t}))\Phi(z_{t-1}(\xbm_{t}))+\sigma_{t-1}(\xbm_{t})\phi(z_{t-1}(\xbm_{t}))+  \beta_t^{1/2} \sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq& (y^+_{t-1}-f(\xbm_{t})+f(\xbm_{t})-\mu_{t-1}(\xbm_{t}))\Phi(z_{t-1}(\xbm_{t}))+0.4\sigma_{t-1}(\xbm_{t})+  \beta_t^{1/2} \sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq& (\beta_t^{1/2}+0.4)\sigma_{t-1}(\xbm_{t})+ \beta_t^{1/2} \sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}, 
  \end{aligned}
  \end{equation}
  where the first line uses Lemma~\ref{lem:EI-compact-rkhs-bound}, the second line uses the definition of $\xbm_t$, and the last line uses Lemma~\ref{lem:EI-bound-RKHS-t-only}, $\Phi(\cdot)<1$, and $y^+_{t-1}-f(\xbm_{t})\leq 0$.
 If $y^+_{t-1}-f(\xbm_{t})> 0$, with probability $\geq 1-\delta$,
   \begin{equation} \label{eqn:EI-instregret-RKHS-pf-2}
  \centering
  \begin{aligned}
        r_t =& f(\xbm_{t})-f(\xbm^*) =  f(\xbm_{t})-y^+_{t-1}+ y^+_{t-1}-f(\xbm^*)\\
              \leq& f(\xbm_{t})-y^+_{t-1}+EI_{t-1}(\bar{\xbm}_{t}^*) + \beta^{1/2}_t\sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\
              \leq& f(\xbm_{t})-y^+_{t-1}+(y^+_{t-1}-f(\xbm_{t})+f(\xbm_{t})-\mu_{t-1}(\xbm_{t}))\Phi(z_{t-1}(\xbm_{t}))\\
                  &+\sigma_{t-1}(\xbm_{t})\phi(z_{t-1}(\xbm_{t}))  + \beta^{1/2}_t\sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\
               \leq&( \beta_t^{1/2}+0.4)\sigma_{t-1}(\xbm_{t})+ \beta^{1/2}_t\sigma_{t-1}(\bar{\xbm}^*_t)+\frac{1}{t^2}. 
  \end{aligned}
  \end{equation}
  The first inequality in~\eqref{eqn:EI-instregret-RKHS-pf-2} is by Lemma~\ref{lem:EI-compact-rkhs-bound}, while the last inequality is due to Lemma~\ref{lem:EI-bound-RKHS-t-only}, Lemma~\ref{lem:phi}, and $y^+_{t-1}-f(\xbm_{t})> 0$. 
   Combine~\eqref{eqn:EI-instregret-RKHS-pf-1} and~\eqref{eqn:EI-instregret-RKHS-pf-2} and the proof is complete.
\end{proof}

\begin{theorem}\label{theorem:EI-regret-rkhs}
Given $\delta\in(0,1)$, let  $\beta_t^{1/2} = c_3 (B+ c_{\alpha}\sqrt{2\log(2\pi_t/\delta)\} + 2 d \log(c_t)}) $, 
where $\sum_{t=1}^{\infty} \pi_t=1$, $c_{\alpha}=\frac{\sigma_{\alpha}}{\sigma}$, $c_t 1+rt^2 L$, and $c_3=1.328$. 
The BO-EI Algorithm~\ref{} has the regret bound
 \begin{equation} \label{eqn:EI-regret-rkhs-1}
  \centering
  \begin{aligned}
     P\left\{ R_T \leq  \frac{1}{2} (0.4+\beta_T^{1/2}) (C_1 T \gamma_T)^{1/2}+ \sum_{t=1}^T  \beta_t^{1/2}\sigma_{t-1}(\xbm^*)+ M_h+2\right\}  \geq 1-\delta,
  \end{aligned}
\end{equation}
for any $T$, where $C_1=8/log(1+\sigma^{-2})$ and $M_h>0$ is a constant. 
\end{theorem}

\begin{proof}
   The posterior variance $\sigma_{t}(\xbm)$ is a Lipschitz continuous function of $\xbm$ and its Lipschitz constant, denoted as $L_{t}^{\sigma}$ is a function of $h_t$, $t$ and the kernel functions. In~\cite{lederer2019uniform} (Theorem 3.1), it is shown that $L_{t}^{\sigma}=\mathcal{O}(\frac{1}{\sqrt{t}})$ as $t\to\infty$ if $h_t=\mathcal{O}(\frac{1}{t^2})$, which is our choice in this section~\eqref{eqn:ht-1}. 

   From Lemma~\ref{lemma:EI-instregret-RKHS} and the choice of $\beta_t$, we have~\eqref{eqn:EI-instregret-RKHS-1} with probability $\geq 1-\delta$. Thus,
 \begin{equation} \label{eqn:EI-regret-rkhs-pf-1}
  \centering
  \begin{aligned}
   r_t \leq& (\beta_t^{1/2}+0.4)\sigma_{t-1}(\xbm_{t}) + \beta^{1/2}_t (\sigma_{t-1}(\xbm^*)+ L_{t}^{\sigma}(h_t) \norm{\bar{\xbm}^*_t-\xbm^*})+\frac{1}{t^2}\\
        \leq& (\beta_t^{1/2}+0.4)\sigma_{t-1}(\xbm_{t}) + \beta^{1/2}_t (\sigma_{t-1}(\xbm^*)+ L_{t}^{\sigma}(h_t) \frac{1}{Lt^2}+\frac{1}{t^2}.\\
   \end{aligned}
\end{equation}
   Clearly, $\sum_{t=1}^{\infty} \beta^{1/2}_t L_{t}^{\sigma}(h_t) \frac{1}{L t^2}<\infty$.
   Define constant $M_h$ so that $\sum_{t=1}^{\infty} \beta^{1/2}_t L_{t}^{\sigma}(h_t) \frac{1}{L t^2}<M_h$.
  
   Using Lemma~\ref{lem:infogain},~\ref{lem:variancebound}, and the Cauchy Schwarz inequality, we know $\sum_{t=1}^T \sigma_{t-1}(\xbm_t) \leq \frac{1}{2} (C_1 T\gamma_T)^{1/2}$, where $C_1=8/\log(1+\sigma^{-2})$. Hence,~\eqref{eqn:EI-regret-rkhs-pf-1} leads to 
 \begin{equation} \label{eqn:EI-regret-rkhs-pf-2}
  \centering
  \begin{aligned}
      R_T =\sum_{t=1}^T r_t \leq \frac{1}{2} (0.4+\beta_T^{1/2}) (C_1 T \gamma_T)^{1/2}+ \sum_{t=1}^T  \beta_t^{1/2}\sigma_{t-1}(\xbm^*)+ M_h+2,
   \end{aligned}
\end{equation}
   with probability $\geq 1-\delta$.
\end{proof}
\begin{remark}\label{remark:eiregret}
 Based on Theorem~\ref{theorem:EI-regret-rkhs}, if $ \sum_{t=1}^T \beta_t^{1/2} \sigma_{t-1}(\xbm^*)= o(T)$, the BO-EI algorithm is a no-regret algorithm with probability $\geq 1-\delta$. However, to the best of our knowledge, the rate of the sum of $\sigma_{t-1}(\xbm^*)$ has not been proven. 
\end{remark}




==> Sections/Vei.tex <==
\section{Variance expected improvement}\label{se:algorithm}
From the convergence analysis, it is clear that EI has strong asymptotoic convergence properties for a large number of functions.
However, its fixed trade-off between exploitation and exploration determined by the nonconvex EI function might not generate a no-regret algorithm. 
In this section, we propose a simple modification to achieve the no-regret properties that might be more preferrable for some applications, as well as improved probability for the asymptotic convergence result. We first point out  that the theoretical bounds are often much larger than actual BO-EI results in practice. Therefore, the proposed algorithm, while enjoying improvement theoretical properties, is not guaranteed for better performance in practice. 

The variance $\sigma_{t}(\xbm^*)$ at the optimal point $\xbm^*$ is one of the main difficulty in our analysis. Therefore, we add an explicit expression of $\sigma_t(\xbm)$ to EI so that exploration is guaranteed to be emphasized as the iteration progresses, which then ensures $\sigma_{t}(\xbm)$ is reduced at any $\xbm\in C$, including $\xbm^*$. 
The modified EI with enhanced exploration is referred to as variance expected improvement (VEI) with the following expression
\begin{equation} \label{eqn:VEI}
 \centering
  \begin{aligned}
       VEI_t(\xbm,\alpha) =   (y_{t}^+-\mu_{t}(\xbm))\Phi(z_{t}(\xbm,\alpha))+\sigma_{t}^{\alpha}(\xbm)\phi(z_{t}(\xbm,\alpha))+\theta \sigma_{t}^{\alpha}(\xbm), 
  \end{aligned}
\end{equation}
where $\alpha\in (0,1]$ and $z_{t}(\xbm,\alpha) = \frac{y_{t}^+-\mu_{t}(\xbm)}{\sigma_{t}^{\alpha}(\xbm)}$.
The explicit standard deviation terms resembles that of UCB. 
We state the convergence theorems for VEI under the GP prior assumptions.
\subsection{VEI under GP prior assumption}\label{se:vei-gp}
In this section, Assumption~\ref{assp:gp} and~\ref{assp:constraint} are valid.
\begin{theorem}\label{theorem:VEI-convg}
   Given $\delta\in(0,1)$, let $\beta=\max\{1, c_{\beta}^{-1} \log (2c_{\alpha}/\delta)\}$ and $\theta\geq \beta^{1/2}$.
   Runing the BO-VEI algorithm with GP prior $(0,k(\xbm,\xbm'))$ leads to the convergence rate 
      \begin{equation} \label{eqn:VEI-convg-star-1}
  \centering
  \begin{aligned}
      r_t  \leq  (2M+2c_\sigma\sigma)\frac{3}{t}+ (0.4+\beta^{1/2}+\theta) \sigma_{t_k}^{\alpha}(\xbm_{t_k+1}))\}, 
   \end{aligned}
  \end{equation} 
  with probability $\geq 1-(\frac{1}{2})^{t/3}-2\Phi(-c_{\sigma})-\delta$.
\end{theorem}
\begin{proof}
   Similar to Theorem~\ref{theorem:EI-convg-star}, we know that with probability $1-2\Phi(-c_{\sigma})$,
  \begin{equation} \label{eqn:VEI-convg-star-pf-1}
  \centering
  \begin{aligned}
        \sum_{t=0}^{T-1}  y^+_{t}-y^+_{t+1} \leq y^+_0 - y_T^+ \leq 2 M +2c_{\sigma}\sigma. 
  \end{aligned}
  \end{equation}
  Therefore, $y^+_{t}-y^+_{t+1} \geq \frac{2M +2c_{\sigma}\sigma}{k}$ at most $k$ times for any $k\in \Nbb$. 
  Let $k=[t/2]$ so that $2k\leq t\leq 2(k+1)$.
  There exists time $k\leq t_k\leq 2k$ so that $y^+_{t_k}-y^+_{t_k+1} < \frac{2M +2c_{\sigma}\sigma}{k}$. 
   Consider first the noiseless case $\sigma=0$.   

  The choice of $\beta$ satisfies Lemma~\ref{lem:IEIbound} and Lemma~\ref{lem:fmu} with $\delta/2$.
  From Lemma~\ref{lem:IEIbound} and $\theta\geq \beta^{1/2}$, with probability $\geq 1-\delta/2$,
  \begin{equation} \label{eqn:VEI-convg-star-pf-2}
  \centering
  \begin{aligned}
          r_t  =& y^+_{t}-f(\xbm^*)\leq y^+_{t_k-1}-f(\xbm^*) = I_{t_k}(\xbm^*)\\
               \leq& EI_{t_k}(\xbm^*,\alpha) + \beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm^*)
               \leq EI_{t_k}(\xbm^*,\alpha) + \theta\sigma_{t_k}^{\alpha}(\xbm^*)
               \leq EI_{t_k}(\xbm_{t_k+1},\alpha) + \theta\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\\
                =& (y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\phi(z_{t_k}(\xbm_{t_k+1},\alpha))  + \theta\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}).\\
             \leq& (y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+0.4\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}) + \theta\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}).
   \end{aligned}
  \end{equation}
    From Lemma~\ref{lem:fmu}, with probability $\geq 1-\delta/2$, 
   \begin{equation} \label{eqn:VEI-convg-star-pf-3}
  \centering
  \begin{aligned}
          y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}) = y^+_{t_k}-f(\xbm_{t_k+1})+f(\xbm_{t_k+1})-\mu_{t_k}(\xbm_{t_k+1}) \leq \frac{2M}{k} +\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}).
    \end{aligned}
  \end{equation}
  Applying~\eqref{eqn:VEI-convg-star-pf-3} to~\eqref{eqn:VEI-convg-star-pf-2}, we have with probability $\geq 1-\delta$, 
  \begin{equation} \label{eqn:VEI-convg-star-pf-6}
  \centering
  \begin{aligned}
          r_t  \leq& \frac{2M}{k}+\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1})+(0.4+\theta)\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}).\\
  \end{aligned}
  \end{equation}

   Next, we consider the noisy case using similar technique as in Theorem~\ref{theorem:EI-convergence-1}. Given a sequence of iterates $\xbm_i$  of size $k\in \Nbb$ where $i\in A_k$, \textit{i.e.}, $|A_k|=k$, the probability of $f(\xbm_i) < y_i = f(\xbm_i)+\epsilon(\xbm_i)$ for all $i\in A_k$ is $(\frac{1}{2})^k$.
   Let $k=[t/3]$ so that $3k\leq t\leq 3(k+1)$.
   There exists $k \leq t_k \leq 3k$ so that $y_{t_k}^+-y_{t_k+1}^+<\frac{2M_f+2c_{\sigma}\sigma}{k}$ and $f(\xbm_{t_k+1})\geq y_{t_k+1}\geq y_{t_k+1}^+$ with probability $\geq 1-(\frac{1}{2})^k$.
 Following the same analysis for the noiseless case   
  with probability $\geq 1-(\frac{1}{2})^k-\delta-2\Phi(-c_{\sigma})$, 
  \begin{equation} \label{eqn:VEI-convg-star-pf-7}
  \centering
  \begin{aligned}
         r_t  \leq& \frac{2M+2c_{\sigma}\sigma}{k}+\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1})+(0.4+ \theta)\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}) .\\
  \end{aligned}
  \end{equation}
  The proof is complete.
\end{proof}

In addition, BO-VEI can be shown to be a no-regret algorithm with our definition of $r_t$.
For brevity of presentation, we use the same discretization $\Cbb_t$ for compact $C$ as in Section~\ref{se:compact}. 
\begin{theorem}\label{thm:VEI-regret}
Given $\delta\in(0,0.698)$, let  $\beta_t = \max\{1,c_{\beta}^{-1}\log ( 2\pi_t c_{\alpha}/\delta)\} + c_{\beta}^{-1} \log(1+rt^2 L) $, where $\pi_t=\frac{\pi^2t^2}{6}$, $c_{\alpha} = 1.09$, and $c_{\beta}=0.427$.
The BO-VEI Algorithm~\ref{} maintains the regret bound
 \begin{equation} \label{eqn:VEI-regbound-1}
  \centering
  \begin{aligned}
     P\left\{ R_T \leq \frac{1}{2} \beta_T^{1/2} ( C_{\gamma} T  \gamma_T)^{1/2}+0.4 \left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}}+2\right\}  \geq 1-\delta,
  \end{aligned}
\end{equation}
for any $T$, where $C_{\gamma}=8/log(1+\sigma^{-2})$. 
\end{theorem}
\begin{proof}
   Notice that the $\beta_t$ in this theorem satisfies the conditions in both  Lemma~\ref{lem:fmu-t} and~\ref{lem:compact-IL} with $\delta/2$. 
  If $y^+_{t}-f(\xbm_{t+1})\leq 0$, with probability greater than $1-\delta$, 
   \begin{equation} \label{eqn:VEI-regbound-pf-1}
  \centering
  \begin{aligned}
          r_t  =& y^+_{t} - f(\xbm^*)  \leq I_t(\xbm^*) 
          \leq EI_t(\bar{\xbm}^*_t,\alpha)  + \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq& EI_t(\bar{\xbm}^*_t,\alpha)  + \theta \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}
          \leq  EI_t^{\alpha}(\xbm_{t+1},\alpha)  + \theta \sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}\\ 
          =& (y^+_{t}-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm),\alpha)+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_t,\alpha))+  \theta \sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}\\ 
          \leq& \beta_t^{1/2}\sigma_{t}(\xbm_{t+1})+(0.4+\theta)\sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}, 
  \end{aligned}
  \end{equation}
  where the first line uses Lemma~\ref{lem:compact-IL}, the second line uses the definition of $\xbm_t$, and the last line uses Lemma~\ref{lem:fmu-t}.
   If $y^+_{t}-f(\xbm_{t+1})> 0$, with probability greater than $1-\delta$,
    \begin{equation} \label{eqn:VEI-regbound-pf-2}
  \centering
  \begin{aligned}
        r_t =& f(\xbm_{t+1})-f(\xbm^*) =  f(\xbm_{t+1})-y^+_{t}+ y^+_{t}-f(\xbm^*)\\
              \leq& f(\xbm_{t+1})-y^+_{t}+EI_{t}(\bar{\xbm}_{t}^*,\alpha) + \beta^{1/2}_t\sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\
                \leq& f(\xbm_{t+1})-y^+_{t}+(y^+_{t}-f(\xbm_{t+1})+f(\xbm_{t+1})-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1},\alpha))\\
                  &+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_{t+1},\alpha))  + \theta \sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}\\
               \leq&\beta_t^{1/2}\sigma_{t}(\xbm_{t+1}) +(0.4+\theta)\sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}, 
  \end{aligned}
  \end{equation}
where the second line uses Lemma~\ref{lem:compact-IL}, the third line uses the definition of $\xbm_{t+1}$, and the last line uses Lemma~\ref{lem:fmu-t}. 


  From Lemma~\ref{lem:variancebound} and Hölder's inequality,~\eqref{eqn:EI-insregret-pf-5} stands.
   Thus, with probability $\geq 1-\delta$
 \begin{equation} \label{eqn:VEI-regbound-pf-3}
  \centering
  \begin{aligned}
      R_T =\sum_{t=1}^Tr_t  \leq (0.4+\theta) \left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}} + \frac{1}{2} (C_{\gamma}T\beta_T\gamma_T)^{1/2}+2,
   \end{aligned}
\end{equation}
   where $C_{\gamma}=8/\log(1+\sigma^{-2})$.
\end{proof}
For commonly used kernels such as squared exponential functions~\cite{srinivas2009gaussian}, BO-VEI algorithm is a no-regret algorithm.

\subsection{VEI under RKHS assumption}\label{se:vei-gp-rkhs}

